A stochastic hybrid model of a biological filter

We present a hybrid model of a biological filter, a genetic circuit which removes fast fluctuations in the cell's internal representation of the extra cellular environment. The model takes the classic feed-forward loop (FFL) motif and represents it as a network of continuous protein concentrations and binary, unobserved gene promoter states. We address the problem of statistical inference and parameter learning for this class of models from partial, discrete time observations. We show that the hybrid representation leads to an efficient algorithm for approximate statistical inference in this circuit, and show its effectiveness on a simulated data set.

==> eptcsdata.tex <==
\providecommand{\firstpage}{100}
\providecommand{\publicationstatus}{Bortolussi, Bujorianu, Pola (Eds.): HAS 2013\\
EPTCS 124, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.124.10}{10.4204/EPTCS.124.10}}

